Tuning Fast Memory Size based on Modeling of Page Migration for Tiered Memory

Tiered memory, built upon a combination of fast memory and slow memory, provides a cost-effective solution to meet ever-increasing requirements from emerging applications for large memory capacity. Reducing the size of fast memory is valuable to improve memory utilization in production and reduce production costs because fast memory tends to be expensive. However, deciding the fast memory size is challenging because there is a complex interplay between application characterization and the overhead of page migration used to mitigate the impact of limited fast memory capacity. In this paper, we introduce a system, Tuna, to decide fast memory size based on modeling of page migration. Tuna uses micro-benchmarking to model the impact of page migration on application performance using three metrics. Tuna decides the fast memory size based on offline modeling results and limited information on workload telemetry. Evaluating with common big-memory applications and using 5% as the performance loss target, we show that Tuna in combination with a page management system (TPP) saves fast memory by 8.5% on average (up to 16%). This is in contrast to the 5% saving in fast memory reported by Microsoft Pond for the same workloads (BFS and SSSP) and the same performance loss target.

==> text/system_abstract_old.tex <==
%\section{System Abstract (1 page)}
\section{Modeling Page Migration}
\label{sec:sys_abs}

Our modeling is based on the following use scenario: the whole memory footprint of the application is allocated in fast memory, but some memory pages can be offloaded to slow memory when they are less frequently accessed, guided by a memory profiling mechanism. By offloading memory pages, the system can save fast memory, but should not lose performance too much (compared with the case of fast memory only). The performance loss threshold $\tau$  is given by the user based on QoS (e.g., $\tau = 5\%$ as in~\cite{10.1145/3575693.3578835}). This use scenario is aligned with the real scenario in a data center~\cite{10.1145/3575693.3578835}.  

We assume that there is a page management system in the above use scenario (e.g., TPP, Thermostat, and Memtis). This system periodically migrates pages between fast memory and slow memory. This period is called the page migration interval. The page migration decision is based on page access frequency in one or multiple time intervals.  We characterize the interaction between page migration and application performance. %as follows.

\begin{itemize}
    \item The page migration competes with the application for memory bandwidth. If the application performance is bounded by memory bandwidth, such a page-migration overhead can lead to large performance loss in the application. 

    \item The application performance can be insensitive to long memory access latency or low memory bandwidth. The performance insensitivity can come from high computation intensity using high instruction-level or thread-level parallelisms. 
\end{itemize}

%To study the impact of page migration on the application performance, we emulate the above interactions using a micro-benchmark. 

When using different fast memory sizes, the page migration happens differently, and the application performance responds differently. We emulate the above interaction using a micro-benchmark, such that we can decide the minimum fast memory size without violating the constraint on performance loss. 

\begin{comment}
\subsection{Characterization of Page Migration} 
From the perspective of page migration, the micro-benchmark should share three characterizations with the application. Within a profiling time interval, %%(denoted by $prof\_int$), 
compared with the application, (1)  the micro-benchmark causes the same number of page migrations between fast memory and slow memory, (2) has the same arithmetic intensity, characterized as attainable floating point operations and integer operations per second (i.e., FLOPS and IOPS), and (3) has the same number of page accesses.

The characterization (1), denoted by $pm$ (including $pm\_de$ and $pm\_pr$ for page demotion and promotion respectively), is necessary to reflect the page migration overhead. The characterizations (2) (denoted by $AI$) and (3) (denoted by $pacc\_f$ and $pacc\_s$ for fast and slow memories respectively) are necessary to model the application sensitivity to memory performance and memory bandwidth consumption from the application respectively.  
\end{comment}


\subsection{Characterization of Page Migration} 
To emulate the interaction between fast memory size and application performance, the micro-benchmark shares two characterizations with the application. Within a profiling time interval, compared with the application, the micro-benchmark (1) has the same arithmetic intensity, characterized as attainable floating point operations and integer operations per second (i.e., FLOPS and IOPS), (2) has the same number of page accesses, and (3) has the same resident set size (RSS).  
%%%and \textcolor{red}{(4) has the similar page migration behaviors for a given fast memory size}. 

The characterizations (1) (denoted by $AI$) and (2) (denoted by $pacc$, including $pacc\_fast$ and $pacc\_slow$ for fast and slow memory accesses respectively) are necessary to model the application sensitivity to memory performance and memory bandwidth consumption from the application respectively. The characterization (3) is needed to model the impact of fast memory size on application performance. 


%%\subsection{Design of Micro-benchmark} 
%%Taking $pacc$, $pm$, $AI$, %%%$prof\_int$ 
%%and the application's resident set size (RSS) as input, the micro-benchmark generates a workload. In essence, the workload performs strided memory accesses to two arrays (one in fast memory and the other in slow memory) whose physical memory consumption are equal to RSS. By mapping array elements to pages, manipulating the stride size to control the number of memory accesses per page, and limiting computation per memory access, we reach the goals of $pacc$, $pm$, and $AI$.

%The micro-benchmark uses the strided memory accesses, because this access pattern allows us to easily bypass the cache hierarchy and control the number of memory accesses at the page level. Note that the micro-benchmark is not designed to exactly follow the memory access patterns of the application. Rather, the micro-benchmark aims to emulate page accesses and migration. From the perspective of page migration on tiered memory, $pacc$, $pm$, and $AI$ determine the performance, and we focus on their impacts and there is no need to model how memory accesses happen (e.g., either using random, stencil, or strided memory access patterns). 


\subsection{Design of Micro-benchmark} 

\textcolor{red}{Based on a ideal modeling of the page management system. }

Taking $pacc$, $AI$, and RSS as input, the micro-benchmark generates a workload. In essence, the workload performs strided memory accesses to two arrays (one in fast memory and the other in slow memory) whose physical memory consumption are equal to RSS. By mapping array elements to pages, manipulating the stride size to control the number of memory accesses per page, and limiting computation per memory access, we reach the goals of $pacc$ and $AI$.

The micro-benchmark uses the strided memory accesses, because this access pattern allows us to easily bypass the cache hierarchy and control the number of memory accesses at the page level. Note that the micro-benchmark is not designed to exactly follow the memory access patterns of the application. Rather, the micro-benchmark aims to emulate page accesses and migrations. From the perspective of page migration on tiered memory, $pacc$, $AI$ and page migration determine the performance on tiered memory, and we focus on their impacts and there is no need to model how memory accesses happen (e.g., either using random, stencil, or strided memory access patterns). 



\textbf{Meeting the requirement on \textit{pacc}.} 
The micro-benchmark allocates at least $NP\_fast$ number of pages and $NP\_slow$ number of pages in fast and slow memories respectively. These pages are accessed once to be physically allocated, as the initialization phase of the micro-benchmark. After that, the micro-benchmark is executed with the page management system in place. 

Given the page promotion threshold in the page management system (i.e.,  $hot\_thr$, the number of memory accesses in a page that can trigger page promotion), $NP\_fast$ and $NP\_slow$ are defined in Equations~\ref{eq:np_fast} and~\ref{eq:np_slow} respectively, and they do not include migrated pages. The pages counted in the two equations are accessed $hot\_thr - 1$ times each. For the migrated pages, their memory accesses are not considered in the two equations, but are considered to meet the requirement on $pm$. Each promoted page is accessed $hot\_thr$ times, and each demoted page is accessed once.

$hot\_thr$ is invariant in some page management systems (e.g., TPP, AutoNUMA, AutoTiering, and M3). But some page management system (e.g., MEMTIS)  dynamically fine-tunes $hot\_thr$ according to the availability of fast memory. For such a dynamic  $hot\_thr$, its value is given as an input when the runtime queries the performance database (see Section~\ref{sec:perf_db}).

\vspace{-15pt}
\begin{align} 
pacc\_fast &= pacc\_fast - pm\_de \times 1 \label{eq:pacc_fast}\\
pacc\_slow &= pacc\_slow - pm\_pr \times hot\_thr \label{eq:pacc_slow}\\
NP\_fast &= pacc\_fast \; / \; (hot\_thr-1) \label{eq:np_fast}\\
NP\_slow &= pacc\_slow \; / \; (hot\_thr-1)  \label{eq:np_slow}
\end{align}
\vspace{-10pt}



\begin{comment}
\textbf{Meeting the requirement on \textit{pacc}.} 
The micro-benchmark allocates at least $NP\_fast$ number of pages and $NP\_slow$ number of pages in fast and slow memories respectively. These pages are accessed once to be physically allocated, as the initialization phase of the micro-benchmark. After that, the micro-benchmark is executed with the page management system in place. 

Given the page promotion threshold in the page management system (i.e.,  $hot\_thr$, the number of memory accesses in a page that can trigger page promotion), $NP\_fast$ and $NP\_slow$ are defined in Equations~\ref{eq:np_fast} and~\ref{eq:np_slow} respectively, and they do not include migrated pages. The pages counted in the two equations are accessed $hot\_thr - 1$ times each. For the migrated pages, their memory accesses are not considered in the two equations, but are considered to meet the requirement on $pm$. Each promoted page is accessed $hot\_thr$ times, and each demoted page is accessed once.

$hot\_thr$ is invariant in some page management systems (e.g., TPP, AutoNUMA, AutoTiering, and M3). But some page management system (e.g., MEMTIS)  dynamically fine-tunes $hot\_thr$ according to the availability of fast memory. For such a dynamic  $hot\_thr$, its value is given as an input when the runtime queries the performance database (see Section~\ref{sec:perf_db}).

\vspace{-15pt}

\begin{align} 
pacc\_fast &= pacc\_fast - pm\_de \times 1 \label{eq:pacc_fast}\\
pacc\_slow &= pacc\_slow - pm\_pr \times hot\_thr \label{eq:pacc_slow}\\
NP\_fast &= pacc\_fast \; / \; (hot\_thr-1) \label{eq:np_fast}\\
NP\_slow &= pacc\_slow \; / \; (hot\_thr-1)  \label{eq:np_slow}
\end{align}

\vspace{-10pt}

\end{comment}




\textbf{Meeting the requirement on \textit{pm}.} The micro-benchmark allocates $pm\_pr$ and $pm\_de$ number of pages in fast memory and slow memory respectively. Each of these $pm\_pr$ pages in slow memory is accessed $hot\_thr$ times, and then promoted to fast memory by the page management system. %After than, each of these $pm\_de$ pages in fast memory is accessed once, and then demoted to slow memory.

To reach of the goal of $pm\_de$, we must consider how page demotion happens. In most of the page management systems, the page demotion (or page reclaim) happens when the free memory space is below a threshold ($free\_page\_thr$). The page demotion is decoupled from the page promotion. To trigger the desired page demotion, the fast memory size is initially set as ($NP\_fast$ + $NP\_slow$ + $pm\_de$ + $pm\_pr$ + $free\_page\_thr$), but is reduced by $pm\_pr$ after all pages are accessed once. The control of fast memory size is implemented by co-running another micro-benchmark which does nothing but allocates physical pages in fast memory to control its available size. 

\textbf{Meeting the requirement on \textit{AI}.} A page access is implemented by loading an array element from main memory. Once the element is loaded, the micro-benchmark performs random floating-point multiplications and integer additions to meet the requirement on AI.

%%%%%\textbf{Meeting the requirement on \textit{prof\_int}.} The micro-benchmark starts a timer to measure the time for page migration, performing arithmetic operations, and memory accesses. The time should be no larger than \textit{prof\_int}, because the micro-benchmark, although performing the same page accesses, does not have overhead (e.g., thread synchronization or control flow) as the application. 

\textbf{Limitation.} memory-level parallelism.
 Distribution of memory accesses across pages.


%%%\textbf{Limitation.} In (1), we do not distinguish fast-to-slow memory migration and slow-to-fast memory migration, based on the assumption that the migrations in two direction share the same memory bandwidth. But some memory (such as Intel Optane as slow memory) has performance asymmetry in load and store accesses. As a result, the migrations in two directions have different bandwidths. To handle this migration performance difference, we can extend our micro-benchmark by differentiating page promotion and demotion. \textcolor{red}{(to discuss more.)}

\subsection{Building and Using Performance Database} 
\label{sec:perf_db}

The performance database collects the execution records of the micro-benchmarks. Each execution record is a set of execution times of the micro-benchmark using various fast memory sizes under a specific configuration. The configuration is a 9-element vector, shown as follows. The execution record is indexed using the configuration. 

\small 
\hspace{10pt} [$pm\_de$, $pm\_pr$, $AI$, $pacc\_fast$, $pacc\_slow$, $prof\_int$, \\ 
\indent \hspace{10pt} $hot\_thr$, $free\_page\_thr$, num\_threads],  
\normalsize

The configuration includes the number of threads to run the micro-benchmark. When multi-threading is used, each thread respects $AI$, and evenly shares $pm$ and $pacc$. The performance database is built offline by exercising various configurations with various fast memory sizes. When multi-threading is used, each thread respects $AI$, and evenly shares $pm$ and $pacc$. 

Once the performance database is built, it can be used at runtime to tune the fast memory size. The runtime periodically measures $pm\_de$, $pm\_pr$, $AI$, $pacc\_fast$, and $pacc\_slow$, and then composes a configuration vector to query the performance database. The execution record whose index is closest to the input configuration vector is returned from the performance database. The runtime use the execution record to choose a minimum fast-memory size whose performance is within a  performance loss target specified by the user. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}

\textcolor{red}{Dr.Li, I am editing my description for the pseudo-code, some grammar needs to change and will be put here later}

To construct the micro-benchmark, we create a very large array $X$, with the length as $wss\_elemts$. The cache line in the testing consists of 8 vector elements, and each vector element is constructed by several array elements from array $X$, in which the number of array elements is determined by the memory data bit in the computer. Array $X$ is being allocated into fast and slow memory. We assume $f$ stands for the proportion of array $X$ allocated in fast memory, and $s$ stands for the proportion of array $X$ allocated in slow memory, which $f+s=1$. When $f=1$, array $X$ is allocated fully in fast memory. When $s=1$, array $X$ is allocated fully in slow memory.

To adapt the feature of the different applications, we use the LLC cache line as one unit to fetch the array page. In the Unix environment, the size of the catchline is $64bytes$, and one catchline can hold 8 vector elements. The unix page size is $4KB$, and one unix page can hold 64 cache lines. we construct the cache line in the following steps.

\begin{algorithm}
	\caption{Load a cache line} \label{loadcacheline}
	\begin{algorithmic}[1] 
  \For{$j=0$ to $7$} 
    \State {$xv_j=$ {$VEC\_FUNC(load,x[sp+(VEC\_ELEMS*j*stride\_size)])$}} 
    \EndFor
\end{algorithmic} 
\end{algorithm}


The model uses stride size to control the distribution of 8 vector elements in memory pages that array $X$ was allocated.

When stride size is small, the 8 vector elements are loaded into the cache line from adjacent pages. When stride size is bigger, the 8 vector elements in the same cache line will be loaded from multiple different pages. For example, when stride size=1, the 8 vector elements in the loaded cache line are from the same page. When stride size=512, since one memory page can include 512 vector elements, the 8 vector elements in the loaded cache line came from 8 continuously adjacent memory pages. With the stride size increasing, the loaded cache line will span wider memory page access. 

Through tracking the Number of Average page accesses $n_{aa}$ from application A by PEBS, the cache line execution time will be repeated $n_{aa}$ times to mimic the application.

Furthermore, in TPP's environment,  $T_p$ is used to represent the promotion threshold. When  $n_{aa} > T_p$, the corresponding slow memory' page will be promoted to fast memory. This performance improvement can be reflected in the results of the micro benchmark.

Micro benchmark is a streaming method, the model will scan the array $X$ from start to end by streaming point $sp$. During each time, one cache line $cl_{sp}$ will be loaded and calculated, then the result vector $rv$ will be stored back to the corresponding pages where its vector elements were loaded. The algorithm is as follows.

\begin{algorithm}
\caption{Micro-benchmark} 
\hspace*{\algorithmicindent} \textbf{Input: array $X$, $f$, $s$ ,$n_{aa}$, $T_P$,  $sp$ is streaming pointer, $WSS\_ELEMS$, $VEC\_ELEMS$,$stride\_size$ }\\
\hspace*{\algorithmicindent} \textbf{Output: results of Micro-benchmark} 
\begin{algorithmic}[1]   
\For{$sp=0$ to  $WSS\_{ELEMS}$, $sp=sp+VEC\_ELEMS*8*stride\_size$} 
\State Repeat $n_{aa}$ time do  
     \State \hspace{0.5cm} Load a catch line $cl_{sp}$ by Algorithm \ref{loadcacheline}
     \State \hspace{0.5cm} Compute  $cl_{sp}$, and get result vector $rv = \left ( rv_{0}, rv_{1}, rv_{3},...,rv_{7} \right)$
     \State \hspace{0.5cm} Store {$rv_{k}$ to {$x[sp+(VEC\_ELEMS*k*stride\_size)]$}} by using $VEC\_FUNC()$,
     \State \hspace{1 cm} where $0\leq k \leq $ 7   
    \State end of repeat
\EndFor 
\end{algorithmic} 
\end{algorithm}

\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> text/tuning_fast_mem_size_old.tex <==
\section{Tuning Fast Memory Size (1 page)}
\label{sec:tuning}


\begin{comment}
\textcolor{red}{ideas of this section are as follows}

1.	How to decide fast memory size based on the performance database.
Through get $pocc_f$ and $pocc_s$, $AI$, $pm$. According to the principle of micro-benchmark, after constructing the performance database, find the corresponding performance, and get the fast memory ratio f, then get the exact fast memory size $sf$.

2.	Set the fast memory size of the application as $sf$.
We need to limit the fast memory size of the application. We can define a memory tuning controller (MTC) (memeater). MTC can dynamically adjust and free the free memory size and then assign the appropriate fast memory to the application. Thus, the application can get the appropriate fast memory (increasing the fast memory size or decreasing the fast memory size based on the passing parameters from the user end).
One example of the work progress is as follows:
When the application (the application is 12 GB) starts, all the consumption is in fast memory. With the given fast memory size by MTC (for example fast memory size =5G), the tpp starts the demotion mechanism to adapt to small fast memory and release free space in fast memory and demote the pages based on LRU strategy (12G consumption will be in slow memory). When the given fast memory size from MTC increases to 6G, the promotion mechanism will adapt to the increase of the fast memory and will bring some hot pages back from slow memory. Inside the memory tunning adapter of the memory management space, by adjusting the free memory size by malloc and unlock the application can get an appropriate fast memory size.

3.	Enable the application to automatically adapt to fast memory size $sf$.
As we know, the original TPP works with the Linux watermark. The watermark mechanism can be enabled and adjusted to suit fast memory size.  To activate TPP demotion, we can recompile and set the Linux min watermark bound as very high (60 percent of the fast memory size) which makes sure TPP will activate demotion.  Then in the Linux system parameter, we can set the min watermark as a high value (45 percent of the fast memory size) which can be adapted to the demotion. Then we can make sure that the TPP demotion and promotion are activated successfully.
\end{comment}

\textbf{Operating System page reclaim}
Inside the Operating System, when physical memory is insufficient, there are three main methods for memory reclaiming which are Background Memory Reclamation (kswapd), Direct Memory Reclaim, and Out of Memory (OOM) Mechanism. kswapd is a kernel thread that is responsible for performing background memory reclamation when there is insufficient physical memory. kswapd operates independently and asynchronously in the background, which can ensure other processes won't be affected and blocked. Inside the kernel, there are three threshold values for capacity which are min watermark, low watermark, and high watermark. 
When the memory exceeds the low water threshold, it indicates the system has sufficient memory, and no memory reclamation is initiated. When the memory falls below the low watermark threshold, it means memory pressure and then kswapd0 will be triggered and activated to start the background memory reclamation until the high watermark is reached. If the memory falls below the min watermark threshold, it indicates user memory is exhausted at this time, which will lead to direct memory reclamation and potential process blocking. To adjust the triggering condition for kswapd, the value of the low watermark threshold needs to be modified. Since the value of the low watermark is achieved based on the min watermark, thus any adjustments involve modifying the value of the min watermark.

\begin{comment}
 The kernel option $/proc/sys/vm/min\_free\_kbytes$ can be used to set and modify the min watermark threshold. 
\end{comment}

Direct Memory reclamation occurs when a process requests memory and the available memory falls below the min watermark. This indicates that the existing memory is insufficient for both memory allocation and the establishment of the mapping relationships. This condition will trigger the direct memory reclamation by blocking the process and starting to reclaim memory concurrently. The drawback of this approach is that blocking processes can lead to extended delays, which will increase CPU utilization and system load. Therefore, the occurrence of direct memory reclamation should be minimized to avoid the potential performance impacts.

After direct memory reclamation, if the remaining free memory in the system is still insufficient for memory allocation, then the Out of Memory (OOM) will be further triggered. The OOM Killer mechanism will terminate a process with high physical memory usage based on the algorithm to free up memory resources. If the physical memory remains insufficient even after killing the process, the OOM Killer will continue to terminate processes with high physical memory usage until enough memory is released.

\textbf{TPP page reclaim}
Inside the Transparent Page Placement for CXL-Enabled Tiered-Memory (TPP), within the user-space environment, the utilization of a tool with a Chameleon-like allows for the identification of page hotness and the facilitation of NUMA migration by user-space APIs, such as $move\_page()$\cite{10.1145/3582016.3582063}. When it comes to detecting the cold pages within the local memory node, the author found that Linux's current LRU-based (Least Recently Used) age management mechanism is not only lightweight but also highly efficient. Integrating LRUs with NUMA Balancing allows for the seamless identification of the majority of hot pages in CXL-Memory, incurring nearly negligible overhead. Linux will try to assign a page to the memory node that corresponds to the CPU where the process is currently in execution. By default, If the local memory node of a CPU reaches its full capacity, the system performs page reclamation by paging out to the swap device. Linux's default LRU-based mechanism is applied to TPP for identifying the demotion candidates. TPP offers a user-space sysctl interface for fine-tuning the aggressiveness of the reclamation process on local nodes and the reclamation on local nodes can be triggered by controlling the free memory threshold through the interface. The default value is empirically set as 2\%, which means when there is only 2\% of the local node's capacity is available for consumption, the reclamation process is triggered.


\begin{comment}
 TPP offers a user-space sysctl  $(/proc/sys/vm/demote\_scale\_factor)$ 
  The default value of $demote\_scale\_factor$ 
\end{comment}

\textbf{Tuning fast memory size}
We built a memory tuning controller (MTC), which has two functions. The first function is about controlling and tuning the free fast memory size in the whole system through the malloc and unmalloc mechanisms. The second function is to dynamically set the size of the application's fast memory by calling the cgroup function based on the user parameters.

\begin{comment}
=========we can just use the first method===================
\end{comment}
1. Adjust fast memory size by the user-specific desired performance loss.

When the application (AP) starts, it is running in fast memory.  MTC uses a memory tuning function to occupy the system memory, this results in less memory available on the system, which triggers the low watermark limit in Linux. Meanwhile, this triggers the demotion mechanism of the TPP. Tpp then demotes the cold pages of AP based on LRU strategy to slow memory and release fast memory of AP until AP is running with a smaller fast memory size. User set a user-specific desired performance loss $l\%$ and memory tuning unit (mtu). MTC repeat occupies fast memory by a mtu and the corresponding AP decreases its’ fast memory by a mtu. In every occupation, the performance loss of AP was calculated by the evaluation formula and the repeat tuning process will finish until the performance loss of AP meets the user-specific performance loss $l \%$.

2. Adjust fast memory size by the user-specific desired fast memory size.

When the application (AP) starts, it is running in fast memory. Setting the fast memory size $s$ of the AP and using MTC's memory tuning function to occupy the system memory, results in less memory available on the system, which will trigger the low watermark limit in the Linux. This will also trigger the demotion mechanism of the TPP. Tpp will then demote the cold pages of AP based on LRU strategy to slow memory and release fast memory of AP until AP is running with $s$ fast memory size.
For increasing the AP’s fast memory size, we set cgroup parameters through MTC to increase the size $s$ of AP’s fast memory and MTC releases some space that MTC occupies. When TPP finds the free space that is released by MTC and starts to promote. Then AP’s hot pages will be promoted to fast memory and AP will adapt to the increased fast memory size. 







